Binary Quantification and Dataset Shift: An Experimental Investigation

Quantification is the supervised learning task that consists of training predictors of the class prevalence values of sets of unlabelled data, and is of special interest when the labelled data on which the predictor has been trained and the unlabelled data are not IID, i.e., suffer from dataset shift. To date, quantification methods have mostly been tested only on a special case of dataset shift, i.e., prior probability shift; the relationship between quantification and other types of dataset shift remains, by and large, unexplored. In this work we carry out an experimental analysis of how current quantification algorithms behave under different types of dataset shift, in order to identify limitations of current approaches and hopefully pave the way for the development of more broadly applicable methods. We do this by proposing a fine-grained taxonomy of types of dataset shift, by establishing protocols for the generation of datasets affected by these types of shift, and by testing existing quantification methods on the datasets thus generated. One finding that results from this investigation is that many existing quantification methods that had been found robust to prior probability shift are not necessarily robust to other types of dataset shift. A second finding is that no existing quantification method seems to be robust enough to dealing with all the types of dataset shift we simulate in our experiments. The code needed to reproduce all our experiments is publicly available at https://github.com/pglez82/quant_datasetshift.

==> tables/concept_table_0.25.tex <==
\begin{tabular}{r|rrrrrr|rrrrrr|rrrrrr}
\toprule
 & \multicolumn{6}{c}{$p_{U}=0.25$} & \multicolumn{6}{c}{$p_{U}=0.5$} & \multicolumn{6}{c}{$p_{U}=0.75$} \\
 & CC & ACC & PCC & PACC & DyS & SLD & CC & ACC & PCC & PACC & DyS & SLD & CC & ACC & PCC & PACC & DyS & SLD \\
\midrule
-2 & \cellcolor{verylightgray} .152 & \cellcolor{verylightgray} .227 & \textbf{\cellcolor{verylightgray} .136} & \cellcolor{verylightgray} .229 & \cellcolor{verylightgray} .219 & \cellcolor{verylightgray} .247 & .048 & .192 & \textbf{.016} & .200 & .183 & .209 & \textbf{.058} & .154 & .108 & .168 & .126 & .135 \\
-1 & \cellcolor{verylightgray} .068 & \cellcolor{verylightgray} .097 & \textbf{\cellcolor{verylightgray} .061} & \cellcolor{verylightgray} .099 & \cellcolor{verylightgray} .086 & \cellcolor{verylightgray} .099 & \textbf{.023} & .095 & .044 & .101 & .080 & .100 & .099 & .092 & .148 & .102 & \textbf{.064} & .076 \\
0 & \ddag{\cellcolor{verylightgray} .016} & \cellcolor{verylightgray} .020 & \textbf{\cellcolor{verylightgray} .012} & \ddag{\cellcolor{verylightgray} .017} & \cellcolor{verylightgray} .017 & \cellcolor{verylightgray} .015 & .069 & .027 & .094 & .026 & \textbf{.020} & .020 & .147 & .033 & .196 & .037 & .021 & \textbf{.020} \\
1 & \dag{\cellcolor{verylightgray} .023} & \cellcolor{verylightgray} .038 & \textbf{\cellcolor{verylightgray} .023} & \cellcolor{verylightgray} .049 & \cellcolor{verylightgray} .051 & \cellcolor{verylightgray} .050 & .110 & \textbf{.045} & .134 & .048 & .067 & .058 & .199 & .053 & .246 & \textbf{.048} & .076 & .057 \\
2 & \ddag{\cellcolor{verylightgray} .042} & \cellcolor{verylightgray} .069 & \textbf{\cellcolor{verylightgray} .042} & \cellcolor{verylightgray} .084 & \cellcolor{verylightgray} .081 & \cellcolor{verylightgray} .081 & .149 & \textbf{.098} & .170 & .103 & .121 & .110 & .258 & .131 & .300 & \textbf{.126} & .153 & \ddag{.128} \\
\bottomrule
\end{tabular}


==> tables/concept_table_0.5.tex <==
\begin{tabular}{r|rrrrrr|rrrrrr|rrrrrr}
\toprule
 & \multicolumn{6}{c}{$p_{U}=0.25$} & \multicolumn{6}{c}{$p_{U}=0.5$} & \multicolumn{6}{c}{$p_{U}=0.75$} \\
 & CC & ACC & PCC & PACC & DyS & SLD & CC & ACC & PCC & PACC & DyS & SLD & CC & ACC & PCC & PACC & DyS & SLD \\
\midrule
-2 & .248 & .241 & .246 & .240 & \textbf{.234} & .239 & \cellcolor{verylightgray} .134 & \cellcolor{verylightgray} .188 & \textbf{\cellcolor{verylightgray} .113} & \cellcolor{verylightgray} .194 & \cellcolor{verylightgray} .192 & \cellcolor{verylightgray} .202 & \textbf{.020} & .132 & .023 & .143 & .126 & .130 \\
-1 & .149 & .100 & .165 & .101 & .095 & \textbf{.090} & \cellcolor{verylightgray} .061 & \cellcolor{verylightgray} .084 & \textbf{\cellcolor{verylightgray} .054} & \cellcolor{verylightgray} .090 & \cellcolor{verylightgray} .087 & \cellcolor{verylightgray} .092 & \textbf{.028} & .067 & .058 & .077 & .064 & .071 \\
0 & .079 & .019 & .105 & \dag{.017} & .016 & \textbf{.015} & \ddag{\cellcolor{verylightgray} .014} & \ddag{\cellcolor{verylightgray} .019} & \textbf{\cellcolor{verylightgray} .010} & \dag{\cellcolor{verylightgray} .017} & \cellcolor{verylightgray} .018 & \dag{\cellcolor{verylightgray} .016} & .074 & .019 & .100 & .020 & .017 & \textbf{.016} \\
1 & \textbf{.039} & .059 & .070 & .072 & .051 & .058 & \cellcolor{verylightgray} .044 & \cellcolor{verylightgray} .064 & \textbf{\cellcolor{verylightgray} .036} & \cellcolor{verylightgray} .067 & \cellcolor{verylightgray} .067 & \cellcolor{verylightgray} .067 & .126 & .068 & .143 & \textbf{.063} & .073 & \ddag{.063} \\
2 & \textbf{.022} & .091 & .054 & .113 & .084 & .089 & \cellcolor{verylightgray} .079 & \cellcolor{verylightgray} .114 & \textbf{\cellcolor{verylightgray} .066} & \cellcolor{verylightgray} .123 & \cellcolor{verylightgray} .121 & \cellcolor{verylightgray} .120 & .181 & .141 & .189 & .138 & .148 & \textbf{.136} \\
\bottomrule
\end{tabular}


==> tables/concept_table_0.75.tex <==
\begin{tabular}{r|rrrrrr|rrrrrr|rrrrrr}
\toprule
 & \multicolumn{6}{c}{$p_{U}=0.25$} & \multicolumn{6}{c}{$p_{U}=0.5$} & \multicolumn{6}{c}{$p_{U}=0.75$} \\
 & CC & ACC & PCC & PACC & DyS & SLD & CC & ACC & PCC & PACC & DyS & SLD & CC & ACC & PCC & PACC & DyS & SLD \\
\midrule
-2 & .327 & .254 & .359 & .249 & .255 & \textbf{.230} & .201 & \textbf{.189} & .215 & .193 & .203 & .196 & \cellcolor{verylightgray} .072 & \cellcolor{verylightgray} .120 & \textbf{\cellcolor{verylightgray} .069} & \cellcolor{verylightgray} .133 & \cellcolor{verylightgray} .128 & \cellcolor{verylightgray} .129 \\
-1 & .227 & .104 & .273 & .102 & .108 & \textbf{.080} & .129 & \textbf{.081} & .154 & .085 & .094 & .085 & \textbf{\cellcolor{verylightgray} .031} & \cellcolor{verylightgray} .056 & \cellcolor{verylightgray} .034 & \cellcolor{verylightgray} .067 & \cellcolor{verylightgray} .066 & \cellcolor{verylightgray} .067 \\
0 & .155 & .029 & .204 & .031 & .022 & \textbf{.020} & .074 & .023 & .101 & .020 & .021 & \textbf{.017} & \cellcolor{verylightgray} .017 & \cellcolor{verylightgray} .019 & \textbf{\cellcolor{verylightgray} .010} & \cellcolor{verylightgray} .016 & \cellcolor{verylightgray} .018 & \cellcolor{verylightgray} .015 \\
1 & .114 & .089 & .162 & .106 & \textbf{.054} & .068 & \textbf{.034} & .082 & .060 & .090 & .064 & .077 & \cellcolor{verylightgray} .050 & \cellcolor{verylightgray} .076 & \textbf{\cellcolor{verylightgray} .042} & \cellcolor{verylightgray} .073 & \cellcolor{verylightgray} .067 & \cellcolor{verylightgray} .072 \\
2 & .102 & .129 & .145 & .156 & \textbf{.088} & .100 & \textbf{.014} & .136 & .032 & .151 & .115 & .134 & \cellcolor{verylightgray} .089 & \cellcolor{verylightgray} .147 & \textbf{\cellcolor{verylightgray} .083} & \cellcolor{verylightgray} .150 & \cellcolor{verylightgray} .137 & \cellcolor{verylightgray} .149 \\
\bottomrule
\end{tabular}


==> tables/conceptv2_table.tex <==
\begin{tabular}{r|rrrrrrr}
\toprule
 & p(y) change & CC & ACC & PCC & PACC & DyS & SLD \\
\midrule
-3 & -0.6 & .591 & \textbf{.579} & .599 & .591 & .604 & .598 \\
-2 & -0.4 & .397 & \textbf{.387} & .402 & .398 & .404 & .401 \\
-1 & -0.2 & .200 & \textbf{.193} & .204 & .200 & .203 & .202 \\
0 & .0 & .022 & .032 & \textbf{.012} & .026 & .027 & .023 \\
1 & .2 & \textbf{.189} & .193 & .198 & .201 & .202 & .198 \\
2 & .4 & \textbf{.385} & .389 & .400 & .405 & .408 & .402 \\
3 & .6 & \textbf{.580} & \dag{.585} & .605 & .613 & .618 & .606 \\
\bottomrule
\end{tabular}


==> tables/prior_results_ACC.tex <==
\begin{table}[H]
\caption{Results for \emph{prior probability shift} for method ACC. In rows, prevalence for the train set; in columns, prevalence for test sample. Mean MAE: 0.059646.}
\label{tab:priorACC}
    \resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
 & 0.00 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 1.00 \\
0.02 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.037 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.142 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.216 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.317 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.362 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.363 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.324 & {\cellcolor[HTML]{F97979}} \color[HTML]{F1F1F1} 0.260 & {\cellcolor[HTML]{F97C7C}} \color[HTML]{F1F1F1} 0.181 & {\cellcolor[HTML]{F79898}} \color[HTML]{000000} 0.098 & {\cellcolor[HTML]{F5C6C6}} \color[HTML]{000000} 0.020 \\
0.10 & {\cellcolor[HTML]{F5BEBE}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.033 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.042 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.051 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.066 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.070 & {\cellcolor[HTML]{F5CBCB}} \color[HTML]{000000} 0.071 & {\cellcolor[HTML]{F5C8C7}} \color[HTML]{000000} 0.055 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.005 \\
0.20 & {\cellcolor[HTML]{F4CFCF}} \color[HTML]{000000} 0.010 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.040 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.044 & {\cellcolor[HTML]{F4D3D3}} \color[HTML]{000000} 0.045 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.006 \\
0.30 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.009 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.029 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.030 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.034 & {\cellcolor[HTML]{F4DDDD}} \color[HTML]{000000} 0.035 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.003 \\
0.40 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.008 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.008 \\
0.50 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.006 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.007 \\
0.60 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.003 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F4D8D8}} \color[HTML]{000000} 0.012 \\
0.70 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.005 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.025 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F4D9D9}} \color[HTML]{000000} 0.012 \\
0.80 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.039 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.038 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F5C4C4}} \color[HTML]{000000} 0.021 \\
0.90 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F6B6B6}} \color[HTML]{000000} 0.078 & {\cellcolor[HTML]{F5C0C0}} \color[HTML]{000000} 0.097 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.079 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.066 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{F4E1E1}} \color[HTML]{000000} 0.050 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.036 & {\cellcolor[HTML]{F4E1E1}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{F5C0C0}} \color[HTML]{000000} 0.022 \\
0.98 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{F7A5A5}} \color[HTML]{000000} 0.096 & {\cellcolor[HTML]{F88C8C}} \color[HTML]{F1F1F1} 0.183 & {\cellcolor[HTML]{F89090}} \color[HTML]{000000} 0.257 & {\cellcolor[HTML]{F88B8B}} \color[HTML]{F1F1F1} 0.308 & {\cellcolor[HTML]{F98080}} \color[HTML]{F1F1F1} 0.341 & {\cellcolor[HTML]{F97A7A}} \color[HTML]{F1F1F1} 0.319 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.263 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.187 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.128 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.050 \\
\end{tabular}
}
\end{table}


==> tables/prior_results_CC.tex <==
\begin{table}[H]
\caption{Results for \emph{prior probability shift} for method CC. In rows, prevalence for the train set; in columns, prevalence for test sample. Mean MAE: 0.144952.}
\label{tab:priorCC}
\begin{tabular}{lccccccccccc}
 & 0.00 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 1.00 \\
0.02 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.012 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{F4D9D9}} \color[HTML]{000000} 0.138 & {\cellcolor[HTML]{F5C1C1}} \color[HTML]{000000} 0.212 & {\cellcolor[HTML]{F7A3A3}} \color[HTML]{000000} 0.287 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.365 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.438 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.515 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.593 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.666 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.742 \\
0.10 & {\cellcolor[HTML]{F4E0E0}} \color[HTML]{000000} 0.109 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.073 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.033 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.048 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{F4D1D1}} \color[HTML]{000000} 0.126 & {\cellcolor[HTML]{F5CBCB}} \color[HTML]{000000} 0.169 & {\cellcolor[HTML]{F5CDCD}} \color[HTML]{000000} 0.204 & {\cellcolor[HTML]{F5CACA}} \color[HTML]{000000} 0.246 & {\cellcolor[HTML]{F5C4C4}} \color[HTML]{000000} 0.290 \\
0.20 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.118 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.088 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.052 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.049 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.084 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.122 & {\cellcolor[HTML]{F4D8D8}} \color[HTML]{000000} 0.151 & {\cellcolor[HTML]{F4D6D6}} \color[HTML]{000000} 0.186 & {\cellcolor[HTML]{F5CECE}} \color[HTML]{000000} 0.227 \\
0.30 & {\cellcolor[HTML]{F4E1E1}} \color[HTML]{000000} 0.108 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.082 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.053 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.061 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.093 & {\cellcolor[HTML]{F4E0E0}} \color[HTML]{000000} 0.117 & {\cellcolor[HTML]{F4DDDD}} \color[HTML]{000000} 0.148 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.181 \\
0.40 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.121 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.096 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.067 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.044 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.075 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.098 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.128 & {\cellcolor[HTML]{F4D9D9}} \color[HTML]{000000} 0.162 \\
0.50 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.139 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.113 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.086 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.055 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.011 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.080 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.111 & {\cellcolor[HTML]{F4DDDD}} \color[HTML]{000000} 0.142 \\
0.60 & {\cellcolor[HTML]{F4D8D8}} \color[HTML]{000000} 0.157 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.131 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.101 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.071 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.046 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.041 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.065 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.096 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.129 \\
0.70 & {\cellcolor[HTML]{F4D6D6}} \color[HTML]{000000} 0.175 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.149 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.119 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.062 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.033 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.053 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.085 & {\cellcolor[HTML]{F4E1E1}} \color[HTML]{000000} 0.119 \\
0.80 & {\cellcolor[HTML]{F5CECE}} \color[HTML]{000000} 0.219 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.189 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.153 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.118 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.088 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.054 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.025 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.046 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.083 & {\cellcolor[HTML]{F4E0E0}} \color[HTML]{000000} 0.120 \\
0.90 & {\cellcolor[HTML]{F5C2C2}} \color[HTML]{000000} 0.292 & {\cellcolor[HTML]{F5C9C9}} \color[HTML]{000000} 0.256 & {\cellcolor[HTML]{F5C9C9}} \color[HTML]{000000} 0.212 & {\cellcolor[HTML]{F5CBCB}} \color[HTML]{000000} 0.167 & {\cellcolor[HTML]{F4D0D0}} \color[HTML]{000000} 0.128 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.085 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.044 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.040 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.086 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.130 \\
0.98 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.737 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.667 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.590 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.511 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.436 & {\cellcolor[HTML]{F97A7A}} \color[HTML]{F1F1F1} 0.359 & {\cellcolor[HTML]{F7A4A4}} \color[HTML]{000000} 0.283 & {\cellcolor[HTML]{F5C3C3}} \color[HTML]{000000} 0.206 & {\cellcolor[HTML]{F4DDDD}} \color[HTML]{000000} 0.130 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.051 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.025 \\
\end{tabular}
\end{table}


==> tables/prior_results_DyS.tex <==
\begin{table}[H]
\caption{Results for \emph{prior probability shift} for method DyS. In rows, prevalence for the train set; in columns, prevalence for test sample. Mean MAE: 0.026866.}
\label{tab:priorDyS}
\begin{tabular}{lccccccccccc}
 & 0.00 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 1.00 \\
0.02 & {\cellcolor[HTML]{F4E1E1}} \color[HTML]{000000} 0.011 & {\cellcolor[HTML]{F4D5D5}} \color[HTML]{000000} 0.030 & {\cellcolor[HTML]{F5C6C6}} \color[HTML]{000000} 0.041 & {\cellcolor[HTML]{F7A8A7}} \color[HTML]{000000} 0.058 & {\cellcolor[HTML]{F88787}} \color[HTML]{F1F1F1} 0.072 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.085 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.097 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.111 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.114 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.104 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.076 \\
0.10 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.005 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F4E1E1}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.033 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.033 & {\cellcolor[HTML]{F4D9D9}} \color[HTML]{000000} 0.019 \\
0.20 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.003 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.025 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.014 \\
0.30 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.004 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.007 \\
0.40 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.006 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.007 \\
0.50 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.006 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.009 \\
0.60 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.005 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.008 \\
0.70 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.007 \\
0.80 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.008 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.006 \\
0.90 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F5C8C7}} \color[HTML]{000000} 0.038 & {\cellcolor[HTML]{F5CCCC}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F4D1D1}} \color[HTML]{000000} 0.034 & {\cellcolor[HTML]{F4D3D3}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{F4DADA}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.007 \\
0.98 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.063 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.087 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.090 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.086 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.080 & {\cellcolor[HTML]{F89090}} \color[HTML]{000000} 0.071 & {\cellcolor[HTML]{F6ADAD}} \color[HTML]{000000} 0.061 & {\cellcolor[HTML]{F5C3C3}} \color[HTML]{000000} 0.051 & {\cellcolor[HTML]{F4D1D1}} \color[HTML]{000000} 0.041 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.030 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.011 \\
\end{tabular}
\end{table}


==> tables/prior_results_PACC.tex <==
\begin{table}[H]
\caption{Results for \emph{prior probability shift} for method PACC. In rows, prevalence for the train set; in columns, prevalence for test sample. Mean MAE: 0.032121.}
\label{tab:priorPACC}
\begin{tabular}{lccccccccccc}
 & 0.00 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 1.00 \\
0.02 & {\cellcolor[HTML]{F5C1C1}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{F6AEAE}} \color[HTML]{000000} 0.056 & {\cellcolor[HTML]{F5CECE}} \color[HTML]{000000} 0.053 & {\cellcolor[HTML]{F4D0D0}} \color[HTML]{000000} 0.049 & {\cellcolor[HTML]{F5C7C7}} \color[HTML]{000000} 0.052 & {\cellcolor[HTML]{F6ACAC}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.074 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.088 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.100 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.078 & {\cellcolor[HTML]{F5C5C5}} \color[HTML]{000000} 0.002 \\
0.10 & {\cellcolor[HTML]{F4D0D0}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.029 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F4CFCF}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F6B1B1}} \color[HTML]{000000} 0.047 & {\cellcolor[HTML]{F6ACAC}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{F7A5A5}} \color[HTML]{000000} 0.069 & {\cellcolor[HTML]{F88181}} \color[HTML]{F1F1F1} 0.073 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.000 \\
0.20 & {\cellcolor[HTML]{F7A7A7}} \color[HTML]{000000} 0.003 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F4D8D8}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F5C7C7}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F5C5C5}} \color[HTML]{000000} 0.043 & {\cellcolor[HTML]{F5C3C3}} \color[HTML]{000000} 0.049 & {\cellcolor[HTML]{F7A4A4}} \color[HTML]{000000} 0.056 & {\cellcolor[HTML]{F4D3D3}} \color[HTML]{000000} 0.002 \\
0.30 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.005 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.025 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F4D8D8}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F4D6D6}} \color[HTML]{000000} 0.036 & {\cellcolor[HTML]{F5C2C2}} \color[HTML]{000000} 0.041 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.001 \\
0.40 & {\cellcolor[HTML]{F88E8E}} \color[HTML]{000000} 0.004 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.025 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F6AFAF}} \color[HTML]{000000} 0.003 \\
0.50 & {\cellcolor[HTML]{F6B0B0}} \color[HTML]{000000} 0.003 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F7A4A4}} \color[HTML]{000000} 0.004 \\
0.60 & {\cellcolor[HTML]{F5C9C9}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F79595}} \color[HTML]{000000} 0.004 \\
0.70 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.030 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.024 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.006 \\
0.80 & {\cellcolor[HTML]{F5CDCD}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{F5BEBE}} \color[HTML]{000000} 0.047 & {\cellcolor[HTML]{F4D6D6}} \color[HTML]{000000} 0.045 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.042 & {\cellcolor[HTML]{F4DDDD}} \color[HTML]{000000} 0.033 & {\cellcolor[HTML]{F4E2E2}} \color[HTML]{000000} 0.025 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F97979}} \color[HTML]{F1F1F1} 0.006 \\
0.90 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{F97F7F}} \color[HTML]{F1F1F1} 0.083 & {\cellcolor[HTML]{F6AFAF}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{F6B8B8}} \color[HTML]{000000} 0.075 & {\cellcolor[HTML]{F5C1C1}} \color[HTML]{000000} 0.056 & {\cellcolor[HTML]{F5C8C8}} \color[HTML]{000000} 0.041 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F4D8D8}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{F5C8C8}} \color[HTML]{000000} 0.038 & {\cellcolor[HTML]{F79797}} \color[HTML]{000000} 0.004 \\
0.98 & {\cellcolor[HTML]{F4DDDD}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.088 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.147 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.142 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.120 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.094 & {\cellcolor[HTML]{F88383}} \color[HTML]{F1F1F1} 0.069 & {\cellcolor[HTML]{F7A0A0}} \color[HTML]{000000} 0.064 & {\cellcolor[HTML]{F6ACAC}} \color[HTML]{000000} 0.064 & {\cellcolor[HTML]{F89090}} \color[HTML]{000000} 0.066 & {\cellcolor[HTML]{F79797}} \color[HTML]{000000} 0.004 \\
\end{tabular}
\end{table}


==> tables/prior_results_PCC.tex <==
\begin{table}[H]
\caption{Results for \emph{prior probability shift} for method PCC. In rows, prevalence for the train set; in columns, prevalence for test sample. Mean MAE: 0.155989.}
\label{tab:priorPCC}
\begin{tabular}{lccccccccccc}
 & 0.00 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 1.00 \\
0.02 & {\cellcolor[HTML]{F6ACAC}} \color[HTML]{000000} 0.357 & {\cellcolor[HTML]{F6B4B4}} \color[HTML]{000000} 0.268 & {\cellcolor[HTML]{F5BDBD}} \color[HTML]{000000} 0.177 & {\cellcolor[HTML]{F5CECE}} \color[HTML]{000000} 0.086 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.005 & {\cellcolor[HTML]{F97A7A}} \color[HTML]{F1F1F1} 0.097 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.187 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.278 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.369 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.460 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.551 \\
0.10 & {\cellcolor[HTML]{F5CACA}} \color[HTML]{000000} 0.246 & {\cellcolor[HTML]{F5CECE}} \color[HTML]{000000} 0.182 & {\cellcolor[HTML]{F4D4D4}} \color[HTML]{000000} 0.115 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.048 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F88989}} \color[HTML]{F1F1F1} 0.086 & {\cellcolor[HTML]{F88F8F}} \color[HTML]{000000} 0.152 & {\cellcolor[HTML]{F89292}} \color[HTML]{000000} 0.220 & {\cellcolor[HTML]{F79696}} \color[HTML]{000000} 0.286 & {\cellcolor[HTML]{F79999}} \color[HTML]{000000} 0.352 & {\cellcolor[HTML]{F79B9B}} \color[HTML]{000000} 0.421 \\
0.20 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.128 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.085 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.039 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F4D1D1}} \color[HTML]{000000} 0.053 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.098 & {\cellcolor[HTML]{F89494}} \color[HTML]{000000} 0.145 & {\cellcolor[HTML]{F79E9E}} \color[HTML]{000000} 0.192 & {\cellcolor[HTML]{F7A7A7}} \color[HTML]{000000} 0.237 & {\cellcolor[HTML]{F6AEAE}} \color[HTML]{000000} 0.283 & {\cellcolor[HTML]{F6B4B4}} \color[HTML]{000000} 0.331 \\
0.30 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.105 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.072 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.035 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.010 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.036 & {\cellcolor[HTML]{F79D9D}} \color[HTML]{000000} 0.071 & {\cellcolor[HTML]{F6ACAC}} \color[HTML]{000000} 0.108 & {\cellcolor[HTML]{F6B3B3}} \color[HTML]{000000} 0.146 & {\cellcolor[HTML]{F6BABA}} \color[HTML]{000000} 0.181 & {\cellcolor[HTML]{F5C3C3}} \color[HTML]{000000} 0.217 & {\cellcolor[HTML]{F5C8C7}} \color[HTML]{000000} 0.256 \\
0.40 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.136 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.105 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.070 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.035 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.010 & {\cellcolor[HTML]{F4D5D5}} \color[HTML]{000000} 0.031 & {\cellcolor[HTML]{F5C8C8}} \color[HTML]{000000} 0.066 & {\cellcolor[HTML]{F5C7C7}} \color[HTML]{000000} 0.102 & {\cellcolor[HTML]{F5CBCB}} \color[HTML]{000000} 0.134 & {\cellcolor[HTML]{F4D1D1}} \color[HTML]{000000} 0.169 & {\cellcolor[HTML]{F4D5D5}} \color[HTML]{000000} 0.207 \\
0.50 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.169 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.139 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.105 & {\cellcolor[HTML]{F4D6D6}} \color[HTML]{000000} 0.070 & {\cellcolor[HTML]{F4DADA}} \color[HTML]{000000} 0.038 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.011 & {\cellcolor[HTML]{F4E0E0}} \color[HTML]{000000} 0.030 & {\cellcolor[HTML]{F4D8D7}} \color[HTML]{000000} 0.065 & {\cellcolor[HTML]{F4D8D8}} \color[HTML]{000000} 0.097 & {\cellcolor[HTML]{F4DCDC}} \color[HTML]{000000} 0.132 & {\cellcolor[HTML]{F4E0E0}} \color[HTML]{000000} 0.168 \\
0.60 & {\cellcolor[HTML]{F4D5D5}} \color[HTML]{000000} 0.209 & {\cellcolor[HTML]{F4D0D0}} \color[HTML]{000000} 0.177 & {\cellcolor[HTML]{F5CACA}} \color[HTML]{000000} 0.141 & {\cellcolor[HTML]{F5C6C6}} \color[HTML]{000000} 0.105 & {\cellcolor[HTML]{F5C4C4}} \color[HTML]{000000} 0.073 & {\cellcolor[HTML]{F5C7C7}} \color[HTML]{000000} 0.041 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.011 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.065 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.101 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.138 \\
0.70 & {\cellcolor[HTML]{F5C6C6}} \color[HTML]{000000} 0.261 & {\cellcolor[HTML]{F5C0C0}} \color[HTML]{000000} 0.228 & {\cellcolor[HTML]{F6B8B8}} \color[HTML]{000000} 0.190 & {\cellcolor[HTML]{F6B0B0}} \color[HTML]{000000} 0.153 & {\cellcolor[HTML]{F7A6A6}} \color[HTML]{000000} 0.118 & {\cellcolor[HTML]{F88E8E}} \color[HTML]{000000} 0.082 & {\cellcolor[HTML]{F4D6D6}} \color[HTML]{000000} 0.045 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.012 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.067 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.106 \\
0.80 & {\cellcolor[HTML]{F6B3B3}} \color[HTML]{000000} 0.331 & {\cellcolor[HTML]{F6ADAD}} \color[HTML]{000000} 0.287 & {\cellcolor[HTML]{F7A8A7}} \color[HTML]{000000} 0.238 & {\cellcolor[HTML]{F7A0A0}} \color[HTML]{000000} 0.188 & {\cellcolor[HTML]{F79696}} \color[HTML]{000000} 0.143 & {\cellcolor[HTML]{F97B7B}} \color[HTML]{F1F1F1} 0.096 & {\cellcolor[HTML]{F4D4D4}} \color[HTML]{000000} 0.048 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.008 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.049 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.097 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.147 \\
0.90 & {\cellcolor[HTML]{F79B9B}} \color[HTML]{000000} 0.418 & {\cellcolor[HTML]{F79898}} \color[HTML]{000000} 0.355 & {\cellcolor[HTML]{F79696}} \color[HTML]{000000} 0.287 & {\cellcolor[HTML]{F89292}} \color[HTML]{000000} 0.220 & {\cellcolor[HTML]{F88E8E}} \color[HTML]{000000} 0.153 & {\cellcolor[HTML]{F88888}} \color[HTML]{F1F1F1} 0.086 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.048 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.114 & {\cellcolor[HTML]{F5CDCD}} \color[HTML]{000000} 0.181 & {\cellcolor[HTML]{F5C9C9}} \color[HTML]{000000} 0.250 \\
0.98 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.548 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.460 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.369 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.278 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.187 & {\cellcolor[HTML]{F97C7C}} \color[HTML]{F1F1F1} 0.095 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.005 & {\cellcolor[HTML]{F5CDCD}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{F5BCBC}} \color[HTML]{000000} 0.177 & {\cellcolor[HTML]{F6B3B3}} \color[HTML]{000000} 0.268 & {\cellcolor[HTML]{F6ACAC}} \color[HTML]{000000} 0.359 \\
\end{tabular}
\end{table}


==> tables/prior_results_SLD.tex <==
\begin{table}[H]
\caption{Results for \emph{prior probability shift} for method SLD. In rows, prevalence for the train set; in columns, prevalence for test sample. Mean MAE: 0.022323.}
\label{tab:priorSLD}
\begin{tabular}{lccccccccccc}
 & 0.00 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 1.00 \\
0.02 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.010 & {\cellcolor[HTML]{F4D0D0}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{F4D4D4}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F5C8C8}} \color[HTML]{000000} 0.043 & {\cellcolor[HTML]{F6B5B5}} \color[HTML]{000000} 0.054 & {\cellcolor[HTML]{F6A9A9}} \color[HTML]{000000} 0.053 & {\cellcolor[HTML]{F88D8D}} \color[HTML]{000000} 0.056 & {\cellcolor[HTML]{F97C7C}} \color[HTML]{F1F1F1} 0.056 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.056 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.016 \\
0.10 & {\cellcolor[HTML]{F4D4D4}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F4D9D9}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F4CFCF}} \color[HTML]{000000} 0.027 & {\cellcolor[HTML]{F4CFCF}} \color[HTML]{000000} 0.026 & {\cellcolor[HTML]{F5CDCD}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F7A2A2}} \color[HTML]{000000} 0.012 \\
0.20 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F4DFDF}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F4DADA}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F4DEDE}} \color[HTML]{000000} 0.021 & {\cellcolor[HTML]{F4DBDB}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F5BCBC}} \color[HTML]{000000} 0.010 \\
0.30 & {\cellcolor[HTML]{F4E0E0}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.008 \\
0.40 & {\cellcolor[HTML]{F3E4E4}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.007 \\
0.50 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3ECEC}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.007 \\
0.60 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EBEB}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.006 \\
0.70 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.014 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.007 \\
0.80 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F3E3E3}} \color[HTML]{000000} 0.020 & {\cellcolor[HTML]{F3E5E5}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3E6E6}} \color[HTML]{000000} 0.022 & {\cellcolor[HTML]{F3E9E9}} \color[HTML]{000000} 0.019 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EDED}} \color[HTML]{000000} 0.016 & {\cellcolor[HTML]{F3EAEA}} \color[HTML]{000000} 0.017 & {\cellcolor[HTML]{F3EEEE}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F3EFEF}} \color[HTML]{000000} 0.013 & {\cellcolor[HTML]{F4E0E0}} \color[HTML]{000000} 0.007 \\
0.90 & {\cellcolor[HTML]{F3F0F0}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{F5CACA}} \color[HTML]{000000} 0.035 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.039 & {\cellcolor[HTML]{F4D2D2}} \color[HTML]{000000} 0.037 & {\cellcolor[HTML]{F4D4D4}} \color[HTML]{000000} 0.034 & {\cellcolor[HTML]{F4D7D7}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F4DDDD}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F4D9D9}} \color[HTML]{000000} 0.023 & {\cellcolor[HTML]{F3E7E7}} \color[HTML]{000000} 0.018 & {\cellcolor[HTML]{F3E8E8}} \color[HTML]{000000} 0.015 & {\cellcolor[HTML]{F4D0D0}} \color[HTML]{000000} 0.009 \\
0.98 & {\cellcolor[HTML]{F3E8E7}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.082 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.111 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.103 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.093 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.081 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.065 & {\cellcolor[HTML]{F97878}} \color[HTML]{F1F1F1} 0.057 & {\cellcolor[HTML]{F6ABAB}} \color[HTML]{000000} 0.038 & {\cellcolor[HTML]{F6BABA}} \color[HTML]{000000} 0.028 & {\cellcolor[HTML]{F79C9C}} \color[HTML]{000000} 0.013 \\
\end{tabular}
\end{table}


==> tables/prior_table_t.tex <==
\begin{tabular}{l|rrrrrrrrrrrrrrrrrrrrr}
\toprule
 & -1.0 & -0.9 & -0.8 & -0.7 & -0.6 & -0.5 & -0.4 & -0.3 & -0.2 & -0.1 & 0.0 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 \\
\midrule
CC & .737 & .479 & .355 & .271 & .213 & .166 & .126 & .091 & .064 & .047 & .035 & .048 & .064 & .092 & .127 & .167 & .213 & .272 & .355 & .478 & .742 \\
ACC & \textbf{.000} & .049 & .088 & .099 & .094 & .086 & .071 & .055 & .041 & .032 & .026 & .034 & .046 & .063 & .077 & .089 & .096 & .095 & .081 & .052 & .020 \\
PCC & .548 & .439 & .352 & .278 & .216 & .162 & .115 & .093 & .085 & .091 & .111 & .090 & .084 & .089 & .112 & .160 & .213 & .276 & .351 & .440 & .551 \\
PACC & .001 & .044 & .077 & .069 & .054 & .042 & .031 & .025 & .023 & .022 & .017 & .021 & .023 & .025 & .029 & .036 & .045 & .053 & .058 & .039 & \textbf{.002} \\
DyS & .063 & \ddag{.053} & \textbf{.045} & \textbf{.040} & \textbf{.032} & \textbf{.028} & \dag{.024} & .021 & .019 & .017 & .016 & .018 & \dag{.019} & .022 & .026 & .030 & .035 & .043 & .053 & .062 & .076 \\
SLD & .001 & \textbf{.041} & .049 & \ddag{.041} & \dag{.034} & \ddag{.029} & \textbf{.023} & \textbf{.020} & \textbf{.017} & \textbf{.015} & \textbf{.014} & \textbf{.017} & \textbf{.018} & \textbf{.020} & \textbf{.022} & \textbf{.024} & \textbf{.025} & \textbf{.027} & \textbf{.030} & \textbf{.029} & .016 \\
\bottomrule
\end{tabular}


==> tables/priorchange_table.tex <==
\begin{tabular}{l|rrrrrr}
\toprule
 & CC & ACC & PCC & PACC & DyS & EMQ \\
\midrule
-0.25 & \textbf{.046} & \ddag{.047} & .066 & \dag{.052} & .102 & .147 \\
-0.20 & \dag{.040} & \textbf{.036} & .055 & \dag{.041} & .066 & .101 \\
-0.15 & .037 & \textbf{.025} & .048 & \ddag{.025} & .036 & .058 \\
-0.10 & .025 & \textbf{.022} & .033 & \ddag{.022} & .026 & .038 \\
-0.05 & \textbf{.017} & .021 & .020 & \ddag{.019} & .021 & \dag{.020} \\
0.00 & .013 & .021 & \textbf{.012} & .018 & .020 & .016 \\
0.05 & \dag{.014} & .025 & \textbf{.013} & .025 & .027 & .029 \\
0.10 & \textbf{.019} & .029 & .023 & .029 & .030 & .037 \\
0.15 & \textbf{.025} & .037 & .034 & .040 & .037 & .051 \\
0.20 & \textbf{.034} & .048 & .046 & .052 & .044 & .062 \\
0.25 & \textbf{.044} & .054 & .060 & .061 & \ddag{.045} & .064 \\
\bottomrule
\end{tabular}

